Introduction to Algogens

This book introduces the concept of Algogens, a promising integration of generative AI with traditional algorithms aimed at improving problem-solving techniques across various fields. It provides an accessible overview of how Algogens combine AI's innovative potential with algorithms' reliability to tackle complex challenges more effectively than either could alone. The text explores the basics of Algogens, their development, applications, and advantages, such as better adaptability and efficiency. Through examples and case studies, readers will learn about Algogens' practical uses today and their potential for future cybersecurity, healthcare, and environmental science innovation. Acknowledging new technologies' challenges and ethical considerations, the book offers a balanced look at the prospects and obstacles facing Algogens. It invites a broad audience, including experts and newcomers, to engage with the topic and consider Algogens' role in advancing our problem-solving capabilities. This work is presented as a starting point for anyone interested in the intersection of AI and algorithms, encouraging further exploration and discussion on this emerging field. It aims to spark curiosity and contribute to the ongoing conversation about how technology can evolve to meet the complex demands of the AI era.

==> latexmkrc <==
$makeindex  = 'makeindex -s StyleInd.ist %O -o %D %S';

# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
